On direct images of pluricanonical bundles

We show that techniques inspired by Koll\'ar and Viehweg's study of weak positivity, combined with vanishing theorems for log-canonical pairs, lead to new consequences regarding generation and vanishing properties for direct images of pluricanonical bundles. We formulate the strongest such results as Fujita conjecture-type statements, which are then shown to govern a range of fundamental properties of direct images of pluricanonical and pluriadjoint line bundles, like effective vanishing theorems, weak positivity, or generic vanishing.

==> macros.tex <==
% Fonts
\usepackage{amsmath,amsfonts,amsthm,mathrsfs}
\usepackage{amssymb}

% Hyperlinks
\usepackage[unicode,bookmarks]{hyperref}
\usepackage[usenames,dvipsnames]{xcolor}
\hypersetup{colorlinks=true,citecolor=NavyBlue,linkcolor=BrickRed,urlcolor=Orange}

% Bibliography
\usepackage[alphabetic,initials]{amsrefs}
\renewcommand{\eprint}[1]{\href{http://www.arxiv.org/abs/#1}{\texttt{#1}}}

%\usepackage{ifthen}

% Enumerate
\usepackage{enumitem}
\newenvironment{renumerate}{%
	\begin{enumerate}[label=(\roman{*}), ref=(\roman{*})]
}{%
	\end{enumerate}%
}
\newenvironment{nenumerate}{%
	\begin{enumerate}[label=(\arabic{*}), ref=(\arabic{*})]
}{%
	\end{enumerate}%
}
\newenvironment{aenumerate}{%
	\begin{enumerate}[label=(\alph{*}), ref=(\alph{*})]
}{%
	\end{enumerate}%
}

% Counters etc.
\usepackage{chngcntr}

% Display keys (disable with option final)
\ifdraft
\usepackage[notcite,notref,color]{showkeys}
\renewcommand*{\showkeyslabelformat}[1]{%
	\mbox{\normalfont\footnotesize\sffamily#1}%
}
\definecolor{labelkey}{gray}{0.5}
\fi

% Improved commutative diagrams
\usepackage{tikz}

\usepackage{tikz-cd}
\tikzset{commutative diagrams/arrow style=math font}

\usetikzlibrary{matrix,arrows}
\newlength{\myarrowsize} 

% Version similar to Computer Modern
\pgfarrowsdeclare{cmto}{cmto}{
	\pgfsetdash{}{0pt} 
	\pgfsetbeveljoin 
	\pgfsetroundcap 
	\setlength{\myarrowsize}{0.6pt}
	\addtolength{\myarrowsize}{.5\pgflinewidth}
	\pgfarrowsleftextend{-4\myarrowsize-.5\pgflinewidth} 
	\pgfarrowsrightextend{.8\pgflinewidth}
}{
	\setlength{\myarrowsize}{0.6pt} 
  	\addtolength{\myarrowsize}{.5\pgflinewidth}  
	\pgfsetlinewidth{0.5\pgflinewidth}
	\pgfsetroundjoin
	% top half
	\pgfpathmoveto{\pgfpoint{1.5\pgflinewidth}{0}}
	\pgfpatharc{-109}{-170}{4\myarrowsize}
	\pgfpatharc{10}{189}{0.58\pgflinewidth and 0.2\pgflinewidth}
	\pgfpatharc{-170}{-115}{4\myarrowsize+\pgflinewidth}
	\pgfpathclose
	\pgfusepathqfillstroke
	% bottom half
	\pgfpathmoveto{\pgfpoint{1.5\pgflinewidth}{0}}
	\pgfpatharc{109}{170}{4\myarrowsize}
	\pgfpatharc{-10}{-189}{0.58\pgflinewidth and 0.2\pgflinewidth}
	\pgfpatharc{170}{115}{4\myarrowsize+\pgflinewidth}
	\pgfpathclose
	\pgfusepathqfillstroke
	% Change line width back
	\pgfsetlinewidth{2\pgflinewidth}
}

\pgfarrowsdeclare{cmonto}{cmonto}{
	\pgfsetdash{}{0pt} 
	\pgfsetbeveljoin 
	\pgfsetroundcap 
	\setlength{\myarrowsize}{0.6pt}
	\addtolength{\myarrowsize}{.5\pgflinewidth}
	\pgfarrowsleftextend{-4\myarrowsize-.5\pgflinewidth} 
	\pgfarrowsrightextend{.8\pgflinewidth}
}{
	\setlength{\myarrowsize}{0.6pt} 
  	\addtolength{\myarrowsize}{.5\pgflinewidth}  
	\pgfsetlinewidth{0.5\pgflinewidth}
	\pgfsetroundjoin
	% top half
	\pgfpathmoveto{\pgfpoint{1.5\pgflinewidth}{0}}
	\pgfpatharc{-109}{-170}{4\myarrowsize}
	\pgfpatharc{10}{189}{0.58\pgflinewidth and 0.2\pgflinewidth}
	\pgfpatharc{-170}{-115}{4\myarrowsize+\pgflinewidth}
	\pgfpathclose
	\pgfusepathqfillstroke
	% bottom half
	\pgfpathmoveto{\pgfpoint{1.5\pgflinewidth}{0}}
	\pgfpatharc{109}{170}{4\myarrowsize}
	\pgfpatharc{-10}{-189}{0.58\pgflinewidth and 0.2\pgflinewidth}
	\pgfpatharc{170}{115}{4\myarrowsize+\pgflinewidth}
	\pgfpathclose
	\pgfusepathqfillstroke
	% top half (2)
	\pgfpathmoveto{\pgfpoint{1.5\pgflinewidth-0.3em}{0}}
	\pgfpatharc{-109}{-170}{4\myarrowsize}
	\pgfpatharc{10}{189}{0.58\pgflinewidth and 0.2\pgflinewidth}
	\pgfpatharc{-170}{-115}{4\myarrowsize+\pgflinewidth}
	\pgfpathclose
	\pgfusepathqfillstroke
	% bottom half (2)
	\pgfpathmoveto{\pgfpoint{1.5\pgflinewidth-0.3em}{0}}
	\pgfpatharc{109}{170}{4\myarrowsize}
	\pgfpatharc{-10}{-189}{0.58\pgflinewidth and 0.2\pgflinewidth}
	\pgfpatharc{170}{115}{4\myarrowsize+\pgflinewidth}
	\pgfpathclose
	\pgfusepathqfillstroke
	% Change line width back
	\pgfsetlinewidth{2\pgflinewidth}
}

\pgfarrowsdeclare{cmhook}{cmhook}{
	\pgfsetdash{}{0pt} 
	\pgfsetbeveljoin 
	\pgfsetroundcap 
	\setlength{\myarrowsize}{0.6pt}
	\addtolength{\myarrowsize}{.5\pgflinewidth}
	\pgfarrowsleftextend{-4\myarrowsize-.5\pgflinewidth} 
	\pgfarrowsrightextend{.8\pgflinewidth}
}{
	\setlength{\myarrowsize}{0.6pt} 
  	\addtolength{\myarrowsize}{.5\pgflinewidth}  
 	\pgfsetdash{}{0pt}
	\pgfsetroundcap
	\pgfpathmoveto{\pgfqpoint{0pt}{-4.667\pgflinewidth}}
	\pgfpathcurveto
    {\pgfqpoint{4\pgflinewidth}{-4.667\pgflinewidth}}
    {\pgfqpoint{4\pgflinewidth}{0pt}}
    {\pgfpointorigin}
	\pgfusepathqstroke
}

% #1 = column sep = 2em
% #2 = row sep = 2.5em
\newenvironment{diagram}[2]{%
\begin{equation}%
\begin{tikzpicture}[>=cmto,baseline=(current bounding box.center),%
	to/.style={-cmto,font=\scriptsize,cap=round},%
	into/.style={cmhook->,font=\scriptsize,cap=round},%
	onto/.style={-cmonto,font=\scriptsize,cap=round},%
	math/.style={matrix of math nodes, row sep=#2, column sep=#1,%
		text height=1.5ex, text depth=0.25ex}]%
}{%
\end{tikzpicture}%
\end{equation}% 
\ignorespacesafterend%
}
\newenvironment{diagram*}[2]{%
\[%
\begin{tikzpicture}[>=cmto,baseline=(current bounding box.center),%
	to/.style={->,font=\scriptsize,cap=round},%
	into/.style={cmhook->,font=\scriptsize,cap=round},%
	onto/.style={-cmonto,font=\scriptsize,cap=round},%
	math/.style={matrix of math nodes, row sep=#2, column sep=#1,%
		text height=1.5ex, text depth=0.25ex}]%
}{%
\end{tikzpicture}%
\]% 
\ignorespacesafterend%
}

% Example of a diagram
% 
% \begin{diagram}{2.5em}{2em}
% \matrix[math] (m) { A & B & C & D \\ }; 
% \path[into] (m-1-1) edge (m-1-2);
% \path[to] (m-1-2) edge node[auto] {$f$} (m-1-3);
% \path[onto] (m-1-3) edge (m-1-4);
% \end{diagram}

% For testing
% \begin{diagram}{2.5em}{2em}
% \matrix[math] (m) { A & \hspace{-1.29em} \raisebox{0.19pt}{$\to$} B \\ };
% \path[to] (m-1-1) edge[red] (m-1-2);
% \end{diagram}


% D-modules and MHM
\newcommand{\MHM}{\operatorname{MHM}}
\newcommand{\MHS}{\operatorname{MHS}}
\newcommand{\DDX}{\mathbb{D}_X}
\newcommand{\DDpt}{\mathbb{D}_{\pt}}
\newcommand{\pt}{\mathit{pt}}
\newcommand{\Dmod}{\mathscr{D}}
\newcommand{\Mmod}{\mathcal{M}}
\newcommand{\Nmod}{\mathcal{N}}
\newcommand{\Ford}[1]{F_{#1}^{\mathrm{ord}}}
\newcommand{\shT}{\mathscr{T}}

% Derived category
\newcommand{\derR}{\mathbf{R}}
\newcommand{\derL}{\mathbf{L}}
\newcommand{\cohH}{\mathcal{H}}
\newcommand{\Ltensor}{\overset{\derL}{\tensor}}
\newcommand{\decal}[1]{\lbrack #1 \rbrack}

\newcommand{\shH}{\mathcal{H}}
\newcommand{\contr}[2]{#1 \lrcorner\, #2}
\newcommand{\Lie}[1]{\mathcal{L}_{#1}}
\newcommand{\pr}{\mathit{pr}}

% Some basic analysis
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\bignorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\biggnorm}[1]{\biggl\lVert#1\biggr\rVert}
\newcommand{\abs}[1]{\lvert #1 \rvert}
\newcommand{\bigabs}[1]{\bigl\lvert #1 \bigr\rvert}
\newcommand{\Bigabs}[1]{\Bigl\lvert #1 \Bigr\rvert}

\newcommand{\eps}{\varepsilon}
\newcommand{\bigpair}[2]{\bigl\langle #1, #2 \bigr\rangle}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}

\newcommand{\tensor}{\otimes}
\newcommand{\del}{\partial}
\newcommand{\delst}{\partial^{\ast}}
\renewcommand{\dbar}{\bar{\partial}}
\newcommand{\dbarst}{\bar{\partial}^{\ast}}
\newcommand{\dz}{\mathit{dz}}
\newcommand{\dzb}{d\bar{z}}


% Spaces
\newcommand{\shExt}{\mathcal{E}\hspace{-1.5pt}\mathit{xt}}
\newcommand{\shTor}{\mathcal{T}\hspace{-2.5pt}\mathit{or}}
\newcommand{\shHom}{\mathcal{H}\hspace{-1pt}\mathit{om}}

% Various sets
\newcommand{\NN}{\mathbb{N}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\QQ}{\mathbb{Q}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\CC}{\mathbb{C}}
\newcommand{\HH}{\mathbb{H}}
\newcommand{\PP}{\mathbb{P}}
\renewcommand{\SS}{\mathbb{S}}

% Derivatives, vector fields etc.
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdert}[2]{\tfrac{\partial #1}{\partial #2}}
\newcommand{\pders}[2]{\partial #1 / \partial #2}
\newcommand{\vfeld}[1]{\frac{\partial}{\partial #1}}
\newcommand{\vfelds}[1]{\partial / \partial #1}


% Sets
\newcommand{\menge}[2]{\bigl\{ \thinspace #1 \thinspace\thinspace \big\vert%
\thinspace\thinspace #2 \thinspace \bigr\}}
\newcommand{\Menge}[2]{\Bigl\{ \thinspace #1 \thinspace\thinspace \Big\vert%
\thinspace\thinspace #2 \thinspace \Bigr\}}
\newcommand{\mengge}[2]{\biggl\{ \thinspace #1 \thinspace\thinspace \bigg\vert%
\thinspace\thinspace #2 \thinspace \biggr\}}
\newcommand{\MENGE}[2]{\left\{ \thinspace #1 \thinspace\thinspace \middle\vert%
\thinspace\thinspace #2 \thinspace \right\}}

% Operators
\DeclareMathOperator{\im}{im}
\DeclareMathOperator{\rk}{rk}
\DeclareMathOperator{\coker}{coker}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\ch}{ch}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\interior}{int}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\Res}{Res}
\DeclareMathOperator{\Spec}{Spec}
\DeclareMathOperator{\Proj}{Proj}
\DeclareMathOperator{\Tor}{Tor}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\grad}{grad}
\renewcommand{\Im}{\operatorname{Im}}
\renewcommand{\Re}{\operatorname{Re}}
\DeclareMathOperator{\Dom}{Dom}
\DeclareMathOperator{\Supp}{Supp}
\DeclareMathOperator{\codim}{codim}
\DeclareMathOperator{\depth}{depth}
\DeclareMathOperator{\rat}{rat}
\DeclareMathOperator{\Cone}{Cone}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\gr}{gr}
\DeclareMathOperator{\DR}{DR}
\DeclareMathOperator{\Spenc}{\widetilde{\mathrm{DR}}}
\DeclareMathOperator{\End}{End}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Ext}{Ext}
\DeclareMathOperator{\GL}{GL}
\DeclareMathOperator{\SL}{SL}
\DeclareMathOperator{\can}{can}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Ch}{Ch}
\DeclareMathOperator{\Alb}{Alb}
\DeclareMathOperator{\Pic}{Pic}
\DeclareMathOperator{\alb}{alb}

\newcommand{\cl}[1]{\overline{#1}}

% Defining terms (in text)
\newcommand{\define}[1]{\emph{#1}}


% Lie algebras
\newcommand{\glie}{\mathfrak{g}}
\newcommand{\hlie}{\mathfrak{h}}
\newcommand{\sltwo}{\mathfrak{sl}_2(\CC)}
\newcommand{\gl}{\mathfrak{gl}}

\newcommand{\lie}[2]{\lbrack #1, #2 \rbrack}
\newcommand{\Biglie}[2]{\Bigl[ #1, #2 \Bigr]}
\newcommand{\bigglie}[2]{\biggl[ #1, #2 \biggr]}
\newcommand{\biglie}[2]{\bigl[ #1, #2 \bigr]}

% Groups
\newcommand{\SU}[1]{\mathrm{SU}(#1)}

% Sheaves
\newcommand{\shf}[1]{\mathscr{#1}}
\newcommand{\OX}{\shf{O}_X}
\newcommand{\OmX}{\Omega_X}
\newcommand{\omegaX}{\omega_X}
\newcommand{\shHO}{\shH_{\shf{O}}}
\newcommand{\shHZ}{\shH_{\ZZ}}
\newcommand{\shHC}{\shH_{\CC}}
\newcommand{\shV}{\shf{V}}
\newcommand{\shVZ}{\shV_{\ZZ}}
\newcommand{\shVO}{\shV_{\shf{O}}}

% Other things
\newcommand{\defeq}{\underset{\textrm{def}}{=}}

\newcommand{\transp}[1]{{#1}^{\dagger}}
\newcommand{\restr}[1]{\big\vert_{#1}}
\newcommand{\Restr}[1]{\bigg\vert_{#1}}

\newcommand{\argbl}{-}

\newcommand{\polring}[2]{ {#1}\lbrack #2 \rbrack }
\newcommand{\powring}[2]{ {#1}\llbracket #2 \rrbracket }

% putting a bar over something (in math mode)
% #2 = shorten the bar by this much
% #3 = move bar to right by this much

\def\overbar#1#2#3{{%
	\setbox0=\hbox{\displaystyle{#1}}%
	\dimen0=\wd0
	\advance\dimen0 by -#2 
	\vbox {\nointerlineskip \moveright #3 \vbox{\hrule height 0.3pt width \dimen0}%
		\nointerlineskip \vskip 1.5pt \box0}%
}}

% Disks etc.
\newcommand{\dst}{\Delta^{\ast}}
\newcommand{\dstn}[1]{(\dst)^{#1}}

% Arrows
\newcommand{\into}{\hookrightarrow}
\newcommand{\onto}{\to\hspace{-0.7em}\to}

% Other commands
\newcommand{\CCpol}{\CC \lbrack t \rbrack}
\newcommand{\inner}[2]{\langle #1, #2 \rangle}
\newcommand{\biginner}[2]{\bigl\langle #1, #2 \bigr\rangle}
\newcommand{\HR}{H_{\RR}}
\newcommand{\HZ}{H_{\ZZ}}
\newcommand{\HC}{H_{\CC}}
\newcommand{\class}[1]{\lbrack #1 \rbrack}
\newcommand{\VC}{V_{\CC}}
\newcommand{\VZ}{V_{\ZZ}}
\newcommand{\Pb}{\bar{P}}
\newcommand{\pil}{\pi_{\ast}}
\newcommand{\jl}{j_{\ast}}
\newcommand{\jlreg}{j_{\ast}^{\mathrm{reg}}}
\newcommand{\jls}{j_{!}}
\newcommand{\jlsl}{j_{!\ast}}
\newcommand{\ju}{j^{\ast}}
\newcommand{\fu}{f^{\ast}}
\newcommand{\fl}{f_{\ast}}
\newcommand{\fus}{f^{!}}
\newcommand{\iu}{i^{\ast}}
\newcommand{\ius}{i^{!}}
\newcommand{\il}{i_{\ast}}
\newcommand{\pu}{p^{\ast}}
\newcommand{\pl}{p_{\ast}}
\newcommand{\qu}{q^{\ast}}
\newcommand{\qus}{q^{!}}
\newcommand{\ou}{o^{\ast}}
\newcommand{\tu}{t^{\ast}}
\newcommand{\tl}{t_{\ast}}
\newcommand{\gu}{g^{\ast}}
\newcommand{\ql}{q_{\ast}}
\newcommand{\piu}{\pi^{\ast}}
\newcommand{\muu}{\mu^{\ast}}
\newcommand{\mul}{\mu_{\ast}}
\newcommand{\fpu}{(f')^{\ast}}
\newcommand{\rhou}{\rho^{\ast}}
\newcommand{\hu}{h^{\ast}}
\newcommand{\varphiu}{\varphi^{\ast}}
\newcommand{\varphil}{\varphi_{\ast}}
\newcommand{\hl}{h_{\ast}}
\newcommand{\fp}{f_{+}}
\newcommand{\hp}{h_{+}}
\newcommand{\gp}{g_{+}}

\newcommand{\IH}{\mathit{IH}}
\newcommand{\Sp}{\operatorname{Sp}}
\newcommand{\DD}{\mathbb{D}}
\newcommand{\psione}[1]{\psi_{#1,1}}
\newcommand{\phione}[1]{\phi_{#1,1}}
\newcommand{\shF}{\shf{F}}
\newcommand{\shG}{\shf{G}}
\newcommand{\shE}{\shf{E}}
\DeclareMathOperator{\Map}{Map}
\newcommand{\shO}{\shf{O}}
\newcommand{\Blog}{\mathcal{B}(\log)}
\newcommand{\DSigma}{D_{\Sigma}}


% Print \subsection numbers in bf
\makeatletter
\let\@@seccntformat\@seccntformat
\renewcommand*{\@seccntformat}[1]{%
  \expandafter\ifx\csname @seccntformat@#1\endcsname\relax
    \expandafter\@@seccntformat
  \else
    \expandafter
      \csname @seccntformat@#1\expandafter\endcsname
  \fi
    {#1}%
}
\newcommand*{\@seccntformat@subsection}[1]{%
  \textbf{\csname the#1\endcsname.}
}
\makeatother

% Print paragraph headings in italic
\makeatletter
\let\@paragraph\paragraph
\renewcommand*{\paragraph}[1]{%
	\vspace{0.3\baselineskip}%
	\@paragraph{\textit{#1}}%
}
\makeatother

% Commands for section numbering
\counterwithin{equation}{subsection}
\counterwithout{subsection}{section}
\counterwithin{figure}{subsection}
\renewcommand{\thesection}{\Alph{section}}

% Number everything consistently
\newtheorem{theorem}[equation]{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{lemma}[equation]{Lemma}
\newtheorem*{lemma*}{Lemma}
\newtheorem{corollary}[equation]{Corollary}
\newtheorem{proposition}[equation]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{conjecture}[equation]{Conjecture}
\newtheorem{variant}[equation]{Variant}
\newtheorem{condition}[equation]{Condition}
\theoremstyle{definition}
\newtheorem{definition}[equation]{Definition}
\newtheorem*{definition*}{Definition}
\theoremstyle{remark}
\newtheorem{remark}[equation]{Remark}
\newtheorem*{assumption}{Assumption}
\newtheorem*{problem}{Problem}
\newtheorem{question}[equation]{Question}
\newtheorem{exercise}{Exercise}[section]
\newtheorem{example}[equation]{Example}
\newtheorem*{example*}{Example}
\newtheorem*{problem*}{Problem}
\newtheorem*{note}{Note}
\newtheorem*{notation}{Notation}
\theoremstyle{plain}



% Nicer hyperlinks
\newcommand{\theoremref}[1]{\hyperref[#1]{Theorem~\ref*{#1}}}
\newcommand{\lemmaref}[1]{\hyperref[#1]{Lemma~\ref*{#1}}}
\newcommand{\definitionref}[1]{\hyperref[#1]{Definition~\ref*{#1}}}
\newcommand{\propositionref}[1]{\hyperref[#1]{Proposition~\ref*{#1}}}
\newcommand{\conjectureref}[1]{\hyperref[#1]{Conjecture~\ref*{#1}}}
\newcommand{\corollaryref}[1]{\hyperref[#1]{Corollary~\ref*{#1}}}
\newcommand{\exampleref}[1]{\hyperref[#1]{Example~\ref*{#1}}}


% Number \figure using equation
\makeatletter
\let\old@caption\caption
\renewcommand*{\caption}[1]{%
	\setcounter{figure}{\value{equation}}%
	\stepcounter{equation}%
	\old@caption{#1}\relax%
}
\makeatother

% For the introduction
\newcounter{intro}
\renewcommand{\theintro}{\Alph{intro}}
\newtheorem{intro-conjecture}[intro]{Conjecture}
\newtheorem{intro-corollary}[intro]{Corollary}
\newtheorem{intro-theorem}[intro]{Theorem}

% Other macros
\newcommand{\OA}{\mathscr{O}_A}
\newcommand{\OmA}{\Omega_A}
\newcommand{\OmB}{\Omega_B}
\newcommand{\Ah}{\hat{A}}
\newcommand{\omY}{\omega_Y}
\newcommand{\omXp}{\omega_{X'}}
\newcommand{\OXp}{\shO_{X'}}
\newcommand{\shB}{\mathcal{B}}
\newcommand{\OmXp}{\Omega_{X'}}
\newcommand{\OmY}{\Omega_Y}
\newcommand{\OY}{\shO_Y}

\newcommand{\df}{\mathit{df}}
\newcommand{\MI}{\mathcal{J}}

% Sectioning
%\newcommand{\newpar}[1]{\subsection{\texorpdfstring{}{}}}
\newcommand{\newpar}{\subsection{}}
\newcommand{\parref}[1]{\hyperref[#1]{\S\ref*{#1}}}

% Nice command for \widebar
\makeatletter
\newcommand*\if@single[3]{%
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}%
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}%
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
%The bar will be moved to the right by a half of \macc@kerna, which is computed by amsmath:
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
%If there's a superscript following the bar, then no negative kern may follow the bar;
%an additional {} makes sure that the superscript is high enough in this case:
\newcommand*\widebar[1]{\@ifnextchar^{{\wide@bar{#1}{0}}}{\wide@bar{#1}{1}}}
%Use a separate algorithm for single symbols:
\newcommand*\wide@bar[2]{\if@single{#1}{\wide@bar@{#1}{#2}{1}}{\wide@bar@{#1}{#2}{2}}}
\newcommand*\wide@bar@[3]{%
  \begingroup
  \def\mathaccent##1##2{%
%If there's more than a single symbol, use the first character instead (see below):
    \if#32 \let\macc@nucleus\first@char \fi
%Determine the italic correction:
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}%
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}%
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
%Now \dimen@ is the italic correction of the symbol.
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
%Now \@tempdima is the width of the symbol.
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
%Now \dimen@ = (italic correction / 3) - (Breite / 10)
    \ifdim\dimen@>\z@ \dimen@0pt\fi
%The bar will be shortened in the case \dimen@<0 !
    \rel@kern{0.6}\kern-\dimen@
    \if#31
      \overline{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}%
      \advance\dimen@0.4\dimexpr\macc@kerna
%Place the combined final kern (-\dimen@) if it is >0 or if a superscript follows:
      \let\final@kern#2%
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      \overline{\rel@kern{-0.6}\kern\dimen@#1}%
    \fi
  }%
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}%
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
%The following initialises \macc@kerna and calls \mathaccent:
  \if#31
    \macc@nested@a\relax111{#1}%
  \else
%If the argument consists of more than one symbol, and if the first token is
%a letter, use that letter for the computations:
    \def\gobble@till@marker##1\endmarker{}%
    \futurelet\first@char\gobble@till@marker#1\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}%
    \fi
    \macc@nested@a\relax111{\first@char}%
  \fi
  \endgroup
}
\makeatother


